SSTM: Spatiotemporal Recurrent Transformers for Multi-frame Optical Flow Estimation

Inaccurate optical flow estimates in and near occluded regions, and out-of-boundary regions are two of the current significant limitations of optical flow estimation algorithms. Recent state-of-the-art optical flow estimation algorithms are two-frame based methods where optical flow is estimated sequentially for each consecutive image pair in a sequence. While this approach gives good flow estimates, it fails to generalize optical flows in occluded regions mainly due to limited local evidence regarding moving elements in a scene. In this work, we propose a learning-based multi-frame optical flow estimation method that estimates two or more consecutive optical flows in parallel from multi-frame image sequences. Our underlying hypothesis is that by understanding temporal scene dynamics from longer sequences with more than two frames, we can characterize pixel-wise dependencies in a larger spatiotemporal domain, generalize complex motion patterns and thereby improve the accuracy of optical flow estimates in occluded regions. We present learning-based spatiotemporal recurrent transformers for multi-frame based optical flow estimation (SSTMs). Our method utilizes 3D Convolutional Gated Recurrent Units (3D-ConvGRUs) and spatiotemporal transformers to learn recurrent space-time motion dynamics and global dependencies in the scene and provide a generalized optical flow estimation. When compared with recent state-of-the-art two-frame and multi-frame methods on real world and synthetic datasets, performance of the SSTMs were significantly higher in occluded and out-of-boundary regions. Among all published state-of-the-art multi-frame methods, SSTM achieved state-of the-art results on the Sintel Final and KITTI2015 benchmark datasets.

==> Tables/kitti.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} ll *{7}{c} }
\cmidrule{1-9} 
 \multirow{2}{*}{\kern20pt Method } &\multirow{2}{*}{Fl-bg \%} &\multirow{2}{*}{Fl-fg \%} &\multirow{2}{*}{Fl-all \%} &\multirow{2}{*}{Fl-bg \%} &\multirow{2}{*}{Fl-fg \%} &\multirow{2}{*}{ Fl-all \%}\\
  &  &   & & &  &  & & & 
 
\cmidrule{1-9}

\kern7pt MFF \cite{ren2019fusion}  & 4.664	& 2.017 &1.222 & 0.893 & 2.902 & 26.810 \\ 

\kern7pt RAFT\cite{teed2020raft} & 3.112 & 1.133 & 0.770 & 0.634 & 1.823 & 16.371\\ 

\kern7pt GMA \cite{jiang2021learning} &  \textbf{2.863} & 1.057 & 0.653 & 0.566 & 1.817 & \textbf{13.492}\\

\kern1pt Ours(SSTM) & - & - & - & - & - & -	\\ 

\kern1pt Ours(SSTM++) & \underline{2.905} & \textbf{0.971} & \underline{0.583} & \textbf{0.510} & \underline{1.678} & \underline{15.045} \\ 

  & 2.959^* & \underline{0.996}^* & \textbf{0.559}^* & \underline{0.515}* & \textbf{1.669}^* & 
 15.117^* \\ 

\cmidrule{1-9}
\end{tabular*} 


==> Tables/trainingSchedule.tex <==
\begin{table}[hbt!]

\setlength\tabcolsep{0pt}
\centering
\caption{ Summary of training schedule. $Loss_1$ and $Loss_2$ refer to loss functions defined in eq. \ref{eq:56} and eq.  \ref{eq:56}. V, S, M, K and HD1k refer to Virtual KITTI2, Sintel, Monkaa, KITTI2015 and HD1k datasets respectively.}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} ll *{8}{c} }
\cmidrule{1-10} 
 \multirow{2}{*}{\kern10pt Stage }
 &\multirow{1.5}{*}{ \kern10pt Training }
 &\multirow{1.5}{*}{Validation}
 &\multirow{1.5}{*}{ Loss}
 &\multirow{2}{*}{Input size}
 &\multirow{1.5}{*}{ Batch}
 &\multirow{1.5}{*}{ Initialized}
 &\multirow{1.5}{*}{Training samples}
 \\
 & \kern23pt data &  data  & function & & size & weights & (triplets)& & &
 
\cmidrule{1-10}

\kern10pt vkitti  & \kern30pt V & V  &  $Loss_1$ & [288, 960] & 8 & - & 38,035\\ 
\kern10pt monkaa & \kern30pt M & S & $Loss_1$ & [456, 720]  & 6 & vkitti &34,384\\
\kern10pt sintel & V+M+S+HD1K  &  S  & $Loss_1$ & [368, 768] & 6 & monkaa & 147,836\\ 
\kern10pt kitti & \kern30pt K &  K  & $Loss_2$ & [288, 960] & 6 & sintel & 200\\ 

\cmidrule{1-10}
\end{tabular*} 
\label{tab:training-stages}
\end{table}
